Ergodicity of Random Walks on Random DFA

Given a DFA we consider the random walk that starts at the initial state and at each time step moves to a new state by taking a random transition from the current state. This paper shows that for typical DFA this random walk induces an ergodic Markov chain. The notion of typical DFA is formalized by showing that ergodicity holds with high probability when a DFA is sampled uniformly at random from the set of all automata with a fixed number of states. We also show the same result applies to DFA obtained by minimizing typical DFA.

==> theorems.tex <==
\section{Our Results}

Let us fix a finite alphabet $\Sigma$ of size $r$. All the results below assume
that $r$ is a constant.
%
Our main result shows that, with probability $1 - o(1)$ when $n \rightarrow
\infty$, a random DFA over $\Sigma$ with $n$ states has a single closed
communicating class, and that this class is aperiodic.
%
Half of this result was already proved in \citep{grusho}.


In view of Grusho's theorem, we only need to show that the closed communicating
class identified by his theorem is aperiodic to prove our result.


Using the definitions in Section~\ref{sec:preliminaries} we can see that the
following result follows immediately from Theorem~\ref{thm:main}.








